Exclusive Chromomagnetism in heavy-to-light FCNCs

We compute matrix elements of the chromomagnetic operator, often denoted by $ {\cal O}_8$, between $B/D$-states and light mesons plus an off-shell photon by employing the method of light-cone sum rules (LCSR) at leading twist-2. These matrix elements are relevant for processes such as $B \to K^* l^+l^-$ and they can be seen as the analogues of the well-known penguin form factors $T_{1,2,3}$ and $f_T$. We find a large CP-even phase for which we give a long-distance (LD) interpretation. We compare our results to QCD factorisation for which the spectator photon emission is end-point divergent. The analytic structure of the correlation function used in our method admits a complex anomalous threshold on the physical sheet. The meaning and handling within the sum rule approach of the anomalous threshold is discussed.

==> table_s_data.tab.tex <==

\begin{tabular}{c|cccc}
$ Q^2 $
& $ G_1^{(\perp)}\times 10^2 $
& $ G_3^{(\parallel)}\times 10^2 $
& $ G_1^{(\perp)}\times 10^2 $
& $ G_3^{(\parallel)}\times 10^2 $
\\ \hline
& $ B^-\rightarrow K^{*-} $
& $ B^-\rightarrow K^{*-} $
& $ \bar B^0\rightarrow\bar K^{*0} $
& $ \bar B^0\rightarrow\bar K^{*0} $
\\ \hline
 $ 0.010 $
& $ 0.2931-0.3960i $
& $ 2.3443+0.8303i $
& $ 0.2022+0.1980i $
& $ -1.1952-0.4151i $
\\ $ 0.261 $
& $ 0.3204-0.3781i $
& $ 1.0673+0.8213i $
& $ 0.1661+0.1890i $
& $ -0.5574-0.4107i $
\\ $ 0.512 $
& $ 0.3384-0.3604i $
& $ 0.7999+0.8122i $
& $ 0.1431+0.1802i $
& $ -0.4243-0.4061i $
\\ $ 0.764 $
& $ 0.3526-0.3429i $
& $ 0.6388+0.8029i $
& $ 0.1251+0.1715i $
& $ -0.3443-0.4014i $
\\ $ 1.015 $
& $ 0.3641-0.3257i $
& $ 0.5217+0.7933i $
& $ 0.1102+0.1629i $
& $ -0.2863-0.3966i $
\\ $ 1.266 $
& $ 0.3736-0.3087i $
& $ 0.4286+0.7834i $
& $ 0.0975+0.1544i $
& $ -0.2403-0.3917i $
\\ $ 1.517 $
& $ 0.3815-0.2920i $
& $ 0.3508+0.7732i $
& $ 0.0866+0.1460i $
& $ -0.2020-0.3866i $
\\ $ 1.768 $
& $ 0.3878-0.2755i $
& $ 0.2834+0.7628i $
& $ 0.0771+0.1378i $
& $ -0.1688-0.3814i $
\\ $ 2.020 $
& $ 0.3929-0.2593i $
& $ 0.2235+0.7519i $
& $ 0.0689+0.1297i $
& $ -0.1395-0.3760i $
\\ $ 2.271 $
& $ 0.3969-0.2434i $
& $ 0.1693+0.7407i $
& $ 0.0617+0.1217i $
& $ -0.1129-0.3703i $
\\ $ 2.522 $
& $ 0.3998-0.2277i $
& $ 0.1196+0.7290i $
& $ 0.0554+0.1139i $
& $ -0.0887-0.3645i $
\\ $ 2.773 $
& $ 0.4018-0.2124i $
& $ 0.0734+0.7168i $
& $ 0.0499+0.1062i $
& $ -0.0662-0.3584i $
\\ $ 3.024 $
& $ 0.4028-0.1974i $
& $ 0.0300+0.7041i $
& $ 0.0453+0.0987i $
& $ -0.0451-0.3521i $
\\ $ 3.275 $
& $ 0.4030-0.1827i $
& $ -0.0110+0.6908i $
& $ 0.0413+0.0913i $
& $ -0.0253-0.3454i $
\\ $ 3.527 $
& $ 0.4024-0.1683i $
& $ -0.0500+0.6768i $
& $ 0.0379+0.0842i $
& $ -0.0064-0.3384i $
\\ $ 4.786 $
& $ 0.3883-0.1024i $
& $ -0.2248+0.5935i $
& $ 0.0295+0.0512i $
& $ 0.0775-0.2967i $
\\ $ 6.046 $
& $ 0.3586-0.0489i $
& $ -0.3754+0.4758i $
& $ 0.0323+0.0245i $
& $ 0.1488-0.2379i $
\\ $ 7.305 $
& $ 0.3177-0.0129i $
& $ -0.4908+0.2946i $
& $ 0.0431+0.0065i $
& $ 0.2019-0.1473i $
\\ $ 8.565 $
& $ 0.2758+0.0000i $
& $ -0.4519+0.0224i $
& $ 0.0562-0.0000i $
& $ 0.1770-0.0112i $
\\ $ 9.824 $
& $ 0.2492+0.0000i $
& $ -0.2972+0.0000i $
& $ 0.0630-0.0000i $
& $ 0.0933-0.0000i $
\\ $ 11.084 $
& $ 0.2312-0.0000i $
& $ -0.2485-0.0000i $
& $ 0.0669+0.0000i $
& $ 0.0613+0.0000i $
\\ $ 12.343 $
& $ 0.2176-0.0000i $
& $ -0.2243-0.0000i $
& $ 0.0696+0.0000i $
& $ 0.0400+0.0000i $
\\ $ 13.603 $
& $ 0.2070-0.0000i $
& $ -0.2128+0.0000i $
& $ 0.0718+0.0000i $
& $ 0.0230-0.0000i $
\\ $ 14.862 $
& $ 0.1986+0.0000i $
& $ -0.2101+0.0000i $
& $ 0.0740-0.0000i $
& $ 0.0076-0.0000i $
\\ $ 16.122 $
& $ 0.1921-0.0000i $
& $ -0.2147-0.0000i $
& $ 0.0763+0.0000i $
& $ -0.0080+0.0000i $
\\ $ 17.381 $
& $ 0.1873-0.0000i $
& $ -0.2267+0.0000i $
& $ 0.0790+0.0000i $
& $ -0.0252-0.0000i $
\\ $ 18.641 $
& $ 0.1843+0.0000i $
& $ -0.2475+0.0000i $
& $ 0.0824-0.0000i $
& $ -0.0459-0.0000i $
\\ $ 19.900 $
& $ 0.1831-0.0000i $
& $ -0.2803+0.0000i $
& $ 0.0869+0.0000i $
& $ -0.0725-0.0000i $
\\ $ 21.160 $
& $ 0.1844-0.0000i $
& $ -0.3310-0.0000i $
& $ 0.0932+0.0000i $
& $ -0.1097+0.0000i $
\\ \hline
& $ D^0\rightarrow\rho^0 $
& $ D^0\rightarrow\rho^0 $
& $ D^+\rightarrow\rho^+ $
& $ D^+\rightarrow\rho^+ $
\\ \hline
 $ 0.010 $
& $ -7.0027-4.9787i $
& $ 14.939+2.507i $
& $ -1.9295+2.4893i $
& $ 19.589-1.254i $
\\ $ 0.048 $
& $ -6.5207-4.7048i $
& $ 10.506+2.673i $
& $ -1.8309+2.3524i $
& $ 0.5204-1.3366i $
\\ $ 0.087 $
& $ -6.2041-4.4945i $
& $ 8.9314+2.7462i $
& $ -1.7662+2.2472i $
& $ -1.0918-1.3731i $
\\ $ 0.125 $
& $ -5.9599-4.3583i $
& $ 7.9497+2.9176i $
& $ -1.7163+2.1792i $
& $ -1.4961-1.4588i $
\\ $ 0.163 $
& $ -5.7571-4.2099i $
& $ 7.2213+3.1650i $
& $ -1.6766+2.1050i $
& $ -1.5870-1.5825i $
\\ $ 0.202 $
& $ -5.5875-4.1273i $
& $ 6.6209+3.4331i $
& $ -1.6417+2.0637i $
& $ -1.5541-1.7166i $
\\ $ 0.240 $
& $ -5.4402-4.0195i $
& $ 6.1014+3.5850i $
& $ -1.6115+2.0098i $
& $ -1.4644-1.7925i $
\\ $ 0.440 $
& $ -4.9159-3.4292i $
& $ 3.7348+4.8267i $
& $ -1.4907+1.7146i $
& $ -0.5866-2.4133i $
\\ $ 0.640 $
& $ -4.6317-3.0393i $
& $ 0.8816+6.7486i $
& $ -1.3979+1.5196i $
& $ 0.8464-3.3743i $
\\ $ 0.840 $
& $ -4.4966-2.6815i $
& $ -3.643+11.193i $
& $ -1.3125+1.3407i $
& $ 3.2215-5.5964i $
\\ $ 1.040 $
& $ -4.4921-2.1974i $
& $ -11.832+18.837i $
& $ -1.2174+1.0987i $
& $ 7.4949-9.4187i $
\\ $ 1.240 $
& $ -4.6038-1.8406i $
& $ -27.338+33.651i $
& $ -1.1080+0.9203i $
& $ 15.490-16.825i $
\\ $ 1.440 $
& $ -4.8063-1.2685i $
& $ -58.743+61.022i $
& $ -0.9925+0.6342i $
& $ 31.511-30.511i $
\end{tabular}


